A Judgmental Construction of Directed Type Theory

We reformulate recent advances in directed type theory--a type theory where the types have the structure of synthetic (higher) categories--as a logical calculus with multiple context 'zones', following the example of Pfenning and Davies. This allows us to have two kinds of variables--'neutral' and 'polar'--with different functoriality requirements. We focus on the lowest-dimension version of this theory (where types are synthetic preorders) and apply the logical language to articulate concepts from the theory of rewriting. We also take the occasion to develop the categorical semantics of dual-context systems, proposing a notion of dual CwF to serve as a common structural base for the model theories of such logics.

==> content/defn/CwF.tex <==
%% content/defn/CwF.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% October 2025
%%
A \keyword{category with families} consists of:
\begin{itemize}
\item a category with terminal object $\Empty$; write $\Con$ for the class of objects (called \enQuote{contexts}) and $\Sub\;\Theta\;\Gamma$ for the set of morphisms (called \enQuote{substitutions}) from $\Theta$ to $\Gamma$;
\item for each $\Gamma\colon\Con$, a set $\Ty\;\Gamma$ of \enQuote{types in context $\Gamma$}, along with a reindexing function $\underlines[\underlines]\colon \Ty\;\Gamma \to \Sub\;\Theta\;\Gamma \to \Ty\;\Theta$ such that $A[\iden]=A$ and $A[\gamma\circ\theta]=A[\gamma][\theta]$;
\item for each $\Gamma\colon\Con$ and $A\colon\Ty\;\Gamma$, a set $\Tm(\Gamma,A)$ of \enQuote{terms of type $A$}, along with a reindexing function $\underlines[\underlines]\colon \Tm(\Gamma,A) \to (\gamma\colon\Sub\;\Theta\;\Gamma) \to \Ty(\Theta,A[\gamma])$ such that $t[\iden]=t$ and $t[\gamma\circ\theta]=t[\gamma][\theta]$;
\item for each $\Gamma\colon\Con$ and $A\colon\Ty\;\Gamma$, a context $\Gamma\cExtend A$ equipped with a substitution $\pp[A]\colon\Sub\;(\Gamma\cExtend A)\;\Gamma$, a \enQuote{variable term} $\vv[A]\colon\Tm(\Gamma\cExtend A,A[\pp[A]])$, and a pairing operation
\[  \underlines,\underlines \colon (\sigma\colon\Sub\;\Theta\;\Gamma) \to \Tm(\Theta, A[\sigma]) \to \Sub\;\Theta\;(\Gamma\cExtend A) \]
such that $\pp[A]\circ (\sigma,s)=\sigma$, $\vv[A][\sigma,s]=s$, $(\sigma,s)\circ \theta = (\sigma\circ\theta,s[\theta])$, and $(\pp[A],\vv[A])=\iden$.
\end{itemize}


==> content/defn/categoryModel.tex <==
%% content/defn/categoryModel.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% October 2025
%%
The \keyword{category model of type theory} is a CwF whose
\begin{itemize}
\item contexts are \textit{categories} and substitutions are functors;
\item types in context $\Gamma$ are families of categories over $\Gamma$;
\item terms in context $\Gamma$ of type $A$ are sections of $A$.
\end{itemize}


==> content/defn/dualCwF.tex <==
%% content/defn/dualCwF.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% October 2025
%%
A \keyword{dual CwF} consists of
\begin{itemize}
\item a category $\mc C$ with a terminal object $\Empty$;
\item a family $\mc D$ of categories over the \textit{opposite} category $\mc C\op$;
\item a section $\bullet$ of $\mc D$ such that $\bullet_\Gamma$ is terminal in $\mc D_\Gamma$ for every $\Gamma\in\mc C$;
\item a CwF structure $(\Ty,\Tm,\cExtend,\ldots)$ on the total category $\smallint\mc D$---write $\Gamma\mid\Delta$ for the pair of $\Gamma$ and $\Delta$---such that the first projections of $(\Gamma\mid\Delta)\cExtend A$ and $\pp[A]$ are $\Gamma$ and $\iden_\Gamma$, respectively.
\end{itemize}


==> content/defn/familySection.tex <==
%% content/defn/familySection.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% October 2025
%%
A \keyword{family of categories} $\mc D$ over a category $\mc C$ consists of
\begin{itemize}
\item a category $\mc D_I$ for each object $I\in\mc C$;
\item a functor $\mc D_j\colon\mc D_I \to \mc D_J$ for every morphism $j\in\mc C(I,J)$ such that $\mc D_{k\circ j}=\mc D_k \circ \mc D_j$ and $\mc D_{\iden_J}$ is the identity functor on $\mc D_J$.
\end{itemize}
\noindent A \keyword{section} $\delta$ of a family $\mc D$ over $\mc C$ assigns
\begin{itemize}
\item objects $I\in\mc C$ to objects $\delta_I\in\mc D_I$ and
\item morphisms $j\in\mc C(I,J)$ to morphisms $\delta_j\in\mc D_J(\mc D_j\;\delta_I, \delta_J)$ such that $\delta_{k\circ j} = \delta_k \circ \mc D_k\;\delta_j$ and $\delta_{\iden_J}=\iden_{\delta_J}$.
\end{itemize}


==> content/defn/syntheticComposition.tex <==
%% content/defn/syntheticComposition.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% October 2025
%%
Define the \keyword{composition of hom-terms}
\[  \Gamma,y::A\mid x\colon A^-,z\colon A, u\colon\hom(x,\pair+ y), v\colon\hom(\pair- y,z) \vdash u\cdot v\colon\hom(x,z) \]
by
\[  u\cdot v := \J[\pm]\;\refl_y. \]


==> content/defn/totalFamCat.tex <==
%% content/defn/totalFamCat.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% October 2025
%%
If $\mc D$ is a \textit{contravariant} family over $\mc C$, that is, a family over $\mc C\op$, then the \keyword{total category} $\smallint\mc D$ of $\mc D$ is the category whose
\begin{itemize}
\item objects are pairs $(I,x)$ where $I\in\mc C$ and $x\in\mc D_I$;
\item morphisms $\smallint\mc D((I,x),(J,y))$ are pairs $(j\in\mc C(I,J), \phi\in\mc D_I(x,\mc D_j\;y))$.
\end{itemize}

